Improving Neural Symbolic Regression with a Diverse Prior and Post-training Alignment

Symbolic regression is the problem of finding an expression that fits a dataset. Solving it requires searching a combinatorial space of candidate expressions. Neural symbolic regression can amortize that search by training a model once on synthetic data and then predicting expressions for a new dataset. But existing models still underperform genetic programming on real, noisy data. We argue that the deficit lies in the training rather than in the paradigm, and present RASR (Reinforced Amortized Symbolic Regression), a method with two key changes to the training recipe. First, we design a synthetic prior that narrows the gap with real-world data: inputs come from the prior of a tabular foundation model; constants are sampled bottom-up, conditioned on the data; targets carry heteroscedastic and structured noise; and everything is standardized. Second, we split training into two stages. Supervised pre-training maximizes the token-level likelihood of a reference expression. This is followed by reinforcement-learning post-training that aligns the model with its inference-time use by rewarding held-out fit and penalizing expression size. On the black-box track of SRBench 2.0, RASR achieves the best mean test $R^2$ rank of all evaluated methods. Three RASR variants, trained with different size penalties, make up most of the accuracy-complexity Pareto front. On Strogatz, our method recovers more ground-truth expressions than any baseline, and on Feynman it is competitive with the best-performing methods.

==> figures/approach/prior-example-values.tex <==
% Generated by notebooks/plot_prior_example_panels.py -- do not edit.
% Values of the single prior draw shown in the pipeline figure.
\newcommand{\PriorCzero}{5.51}%
\newcommand{\PriorCzeroTokA}{5}%
\newcommand{\PriorCzeroTokB}{5}%
\newcommand{\PriorCzeroTokC}{1}%
\newcommand{\PriorCzeroTokExpSign}{e+}%
\newcommand{\PriorCzeroTokExpDigit}{0}%
\newcommand{\PriorCone}{1.36}%
\newcommand{\PriorConeTokA}{1}%
\newcommand{\PriorConeTokB}{3}%
\newcommand{\PriorConeTokC}{6}%
\newcommand{\PriorConeTokExpSign}{e+}%
\newcommand{\PriorConeTokExpDigit}{0}%
\newcommand{\PriorMu}{1.66}%
\newcommand{\PriorMuTokA}{1}%
\newcommand{\PriorMuTokB}{6}%
\newcommand{\PriorMuTokC}{6}%
\newcommand{\PriorMuTokExpSign}{e+}%
\newcommand{\PriorMuTokExpDigit}{0}%
\newcommand{\PriorSigma}{0.29}%
\newcommand{\PriorSigmaTokA}{2}%
\newcommand{\PriorSigmaTokB}{9}%
\newcommand{\PriorSigmaTokC}{0}%
\newcommand{\PriorSigmaTokExpSign}{e-}%
\newcommand{\PriorSigmaTokExpDigit}{1}%

